How to Reduce Temporal Cliques to Find Sparse Spanners

Many real-world networks, such as transportation or trade networks, are dynamic in the sense that the edge set may change over time, but these changes are known in advance. This behavior is captured by the temporal graphs model, which has recently become a trending topic in theoretical computer science. A core open problem in the field is to prove the existence of linear-size temporal spanners in temporal cliques, i.e., sparse subgraphs of complete temporal graphs that ensure all-pairs reachability via temporal paths. So far, the best known result is the existence of temporal spanners with $\mathcal{O}(n\log n)$ many edges. We present significant progress towards proving that linear-size temporal spanners exist in all temporal cliques. We adapt techniques used in previous works and heavily expand and generalize them to provide a simpler and more intuitive proof of the $\mathcal{O}(n\log n)$ bound. Moreover, we use our novel approach to show that a large class of temporal cliques, called edge-pivot graphs, admit linear-size temporal spanners. To contrast this, we investigate other classes of temporal cliques that do not belong to the class of edge-pivot graphs. We introduce two such graph classes and we develop novel techniques for establishing the existence of linear temporal spanners in these graph classes as well.

==> chapters/future-work.tex <==
\section*{Future Work}
Even though we could not solve the overall question to prove that linear spanners exist for temporal bi-cliques, we strongly believe that this conjecture holds true. Therefore, we here list some directions future work can take towards this result:

\begin{itemize}
	\item For now, pivotability, non-revertibleness of edges and swarm vertices are distinct concepts that are each needed to solve another class of artificially constructed graphs. We are currently not aware of graphs that cannot be solved by these techniques. One can follow this path and look for examples which cannot be currently solved, thus either proving the completeness of the necessary techniques or having a counterexample (and most possibly a lead on how to extend the techniques necessary to solve those instances).
	\item When given a ring-shifted graph and adding $+1$ or $-1$ to some edge labels, one gets a graph that has highly pivotable edges. Until now, we could not use this insight to find more conditions on graphs that we can currently solve. In general, having a more detailed overview how our techniques interplay could turn out useful.
\end{itemize}

